From Pointwise to Powerhouse: Initialising Neural Networks with Generative Models

Traditional initialisation methods, e.g. He and Xavier, have been effective in avoiding the problem of vanishing or exploding gradients in neural networks. However, they only use simple pointwise distributions, which model one-dimensional variables. Moreover, they ignore most information about the architecture and disregard past training experiences. These limitations can be overcome by employing generative models for initialisation. In this paper, we introduce two groups of new initialisation methods. First, we locally initialise weight groups by employing variational autoencoders. Secondly, we globally initialise full weight sets by employing graph hypernetworks. We thoroughly evaluate the impact of the employed generative models on state-of-the-art neural networks in terms of accuracy, convergence speed and ensembling. Our results show that global initialisations result in higher accuracy and faster initial convergence speed. However, the implementation through graph hypernetworks leads to diminished ensemble performance on out of distribution data. To counteract, we propose a modification called noise graph hypernetwork, which encourages diversity in the produced ensemble members. Furthermore, our approach might be able to transfer learned knowledge to different image distributions. Our work provides insights into the potential, the trade-offs and possible modifications of these new initialisation methods.

==> 999oldFigures.tex <==
% Figure of the two convergence trajectories next to each other 
\begin{figure*}[t]
    \centering
    \begin{subfigure*}
        \centering
        \includegraphics[width =0.45\textwidth]{Figures/pcam_ACC_Val.pdf}
    \end{subfigure*}
    \begin{subfigure*}
        \centering
        \includegraphics[width =0.45\textwidth]{Figures/cifar_ACC_Val.pdf}
    \end{subfigure*}    
    \caption{Convergence trajectories of the validation accuracy for the different initialisation methods on the PatchCamelyon dataset  over the whole training. Left: Patch Camelyon dataset. Right: CIFAR-10 dataset }
\label{fig:val_conv}
\end{figure*}

% Figure of the two tables of convergence speed next to each other 
\begin{table*}
    \centering
    \begin{subtable}[t]{0.45\linewidth}
            \centering
            \begin{tabular}{l|c|c}
                \multirow{2}{*}{Initialisation} & \multicolumn{2}{l}{Eval steps to reach} \\\cline{2-3}
                    & \hspace*{2mm}    $0.80$ \hspace*{2mm}  & \hspace*{2mm}  $0.85$ \hspace*{2mm}  \\
                 \hline
                 Xavier   & $5$    &$17$\\
                 He & $7$ &$17$\\
                 CVAE & $9$&$20$\\
                 VQVAE* & $5$&$16$\\
                 GHN & $1$&$6$\\
                 Noise GHN & $1$&$3$
            \end{tabular}
            \caption{Number of evaluation steps after which an accuracy of $0.8$, respectively $0.85$ is reached on the PatchCamelyon dataset.}
            \label{tab:val_conv_pcam}
        \end{subtable}
        \begin{subtable}[t]{0.45\linewidth}
            \centering
            \begin{tabular}{l|c|c}
                \multirow{2}{*}{Initialisation} & \multicolumn{2}{l}{Eval steps to reach} \\\cline{2-3}
                    & \hspace*{2mm}    $0.65$ \hspace*{2mm}  & \hspace*{2mm}  $0.75$ \hspace*{2mm}  \\
                 \hline
                 Xavier   &$ 4 $   &$7$\\
                 He &$ 3$ &$7$\\
                 VAE & $3$&$8$\\
                 VQVAE* & $3$&$8$\\
                 GHN & $1$&$4$\\
                 Noise GHN & $1$&$3$
            \end{tabular}
            \caption{Number of evaluation steps after which an accuracy of $0.65$, respectively $0.75$ is reached on the CIFAR-10 dataset.}
            \label{tab:val_conv_cifar}
        \end{subtable}
    \caption{Caption}
    \label{fig:my_label}
\end{table*}

% Figure of Trajectory and Table next to each other 
\begin{figure*}
  \centering
  \begin{subcaptiongroup}
    \centering
    \parbox[b]{.49\linewidth}{%
    \centering
    \includegraphics[width=\linewidth]{Figures/pcam_ACC_Val.pdf}
    \caption{Validation accuracy over the whole training}
    \label{fig:pcam_conv_traj}}%
    \parbox[b]{.49\textwidth}{%
    \centering
    \begin{tabular}{l|c|c}
                \multirow{2}{*}{Initialisation} & \multicolumn{2}{l}{Eval steps to reach} \\\cline{2-3}
                    & \hspace*{2mm}    $0.80$ \hspace*{2mm}  & \hspace*{2mm}  $0.85$ \hspace*{2mm}  \\
                 \hline
                 Xavier   & $5$    &$17$\\
                 He & $7$ &$17$\\
                 CVAE & $9$&$20$\\
                 VQVAE* & $5$&$16$\\
                 GHN & $1$&$6$\\
                 Noise GHN & $1$&$3$
            \end{tabular}
            \vspace{1cm}
    \caption{Number of evaluation steps after which an accuracy of $0.8$, respectively $0.85$ is reached}
    \label{fig:pcam_conv_table}}%
  \end{subcaptiongroup}
  \caption{Convergence trajectories of the validation accuracy for the different initialisation methods on the PatchCamelyon dataset.}\label{fig:pcam_conv}
\end{figure*}

Kapitel 2 
% On the other side, assuming more complex distributions is possible as well, as done in models like the Topographic VAE (TVAE)\cite{keller2021topographic}. For the TVAE, Gaussian distributions are combined facilitating a more strictly structured latent space. 
% Many more variations exist 
% \subsection{Vector Quantized Variational Autoencoders}
% Typically the latent space of VAEs is continuous. 
% However, for some data, such as language or images, a discrete latent space can be a potentially more natural fit \cite{van2017neural}. Additionally, 
% However, a discrete latent space can encourage a model to learn an even more structured latent space since it has to find a way to deal with the limited, even finite, capacity of its latent space.\\
% In order to learn a discrete latent space, we use a technique called \textit{Vector Quantisation} (VQ), where the continuous outputs of the encoder network $\textbf{z}_e$ are mapped onto their corresponding points $\textbf{z}_q$ in the discrete latent space using a codebook $\textbf{e}$. Thus this model is called Vector Quantised Variational Autoencoder (VQVAE).\\ 
% As a projection does not allow for the calculation of gradients, we copy the gradients of the codebook vectors $\textbf{e}_i$ onto the ones for the encoder outputs $\textbf{z}_e$. This approach is called the straight-through estimator \cite{van2017neural}, which he we denote as $$. \\
% In order to learn the codebook, we include a codebook loss $\textbf{L}_C$:
% \begin{equation*}
%     \textbf{L}_C (\textbf{x}) = \frac{1}{K} \sum_{i=1}^K \left [ \norm{sg[\textbf{z}_e] - \textbf{e}_i}_2^2 + \beta \norm{\textbf{z}_e - sg[\textbf{e}_i]}_2^2 \right ],
% \end{equation*}
% where $K$ denotes the size of the codebook, $\beta$ a hyperparamter called the commitment-cost, $\norm{\cdot}$ the $l_2$ norm and $sg$ the stop-gradient operator. The first term moves the codebook vectors towards the outputs of the encoder, while the second term encourages the encoder to produce outputs that are close to the codebook.\\ 
% The VQVAE is then optimized by maximizing
% \begin{equation*}
%     L (\textbf{x})= \log p_{ \boldsymbol \theta}(\textbf{x}|\textbf{z}_q) + \textbf{L}_C (\textbf{x})
% \end{equation*}
% As proposed by the authors of the VQVAE, we involve an autoregressive model $K_{\boldsymbol \Psi}(\textbf{Z})$ with parameters $\boldsymbol \Psi$ called PixelCNN \cite{van2016conditional} for the generation of new samples $\textbf{x}$ from the target distribution $P(\textbf{X})$. We first train it on the quantised outputs of the encoder $\textbf{z}_q$ collected during training. Afterwards we obtain samples from the latent space $\textbf{z}$ from the autoregressive model $K_{\boldsymbol \Psi}(\textbf{Z})$, which we feed into the decoder $P_{ \boldsymbol \theta}(\textbf{X}|\textbf{Z})$.
% % \begin{align*}
% %     \textbf{z} &\sim K_{\boldsymbol \Psi}(\textbf{Z}) \\
% %     \textbf{x} &\sim P_{ \boldsymbol \theta}(\textbf{X}|\textbf{z}).
% % \end{align*} 
